Testing Piketty's Hypothesis on the Drivers of Income Inequality: Evidence from Panel VARs with Heterogeneous Dynamics

Thomas Piketty's Capital in the Twenty-First Century puts forth a logically consistent explanation for changes in income and wealth inequality patterns. However, while rich in data, the book provides no formal empirical testing for its theorized causal chain. This paper tests the hypothesis that the $r-g$ gap drives income inequality and the increasing capital share of national income. Using panel VAR models with data from 18 advanced economies over 30 years, I find no empirical support for Piketty's predictions. The results suggest that dynamics such as savings-rate adjustments and diminishing returns to capital play critical roles in offsetting the hypothesized effects. These findings challenge the theoretical underpinnings of the growth in inequality and call for alternative explanations.

==> archive/lagrobustness.tex <==
The methodology used in the baseline lets the lag-length to be country-specific, making sure that residuals for each of the individual VARs approximate white noise. This contrasts with traditional panel methods, which impose the same lag-length for all panel members. For such reason, I check if the results are consistent even without allowing for lag-length heterogeneity. The alternative specification for models 1 and 3 make sure that all countries use just one lag on the right-hand side. Despite expected changes in the shape of the impulse responses, the results are qualitatively consistent, as seen in Figure \ref{fig:robustness2}.


\begin{figure}[ht] 
\begin{center}
    \includegraphics[scale=0.65]{robustness2.pdf}
\end{center}
\caption[Robustness checks, different lag-lengths]{\textbf{Robustness checks, different lag-lengths - re-estimation of models 1 and 3: Median composite responses}. This figure compares median responses across a distribution of IRFs of 19 countries using different specifications.}\label{fig:robustness2}
\end{figure}

